Contrastive Novelty-Augmented Learning: Anticipating Outliers with Large Language Models

In many task settings, text classification models are likely to encounter examples from novel classes on which they cannot predict correctly. Selective prediction, in which models abstain on low-confidence examples, provides a possible solution, but existing models are often overly confident on unseen classes. To remedy this overconfidence, we introduce Contrastive Novelty-Augmented Learning (CoNAL), a two-step method that generates OOD examples representative of novel classes, then trains to decrease confidence on them. First, we generate OOD examples by prompting a large language model twice: we prompt it to enumerate relevant novel classes, then generate examples from each novel class matching the task format. Second, we train a classifier with a novel contrastive objective that encourages lower confidence on generated OOD examples than training examples. When trained with CoNAL, classifiers improve in their ability to detect and abstain on novel class examples over prior methods by an average of 2.3% in terms of accuracy under the accuracy-coverage curve (AUAC) and 5.5% AUROC across 4 NLP datasets, with no cost to in-distribution accuracy.

==> sections/90-statements.tex <==
\section*{Reproducibility Statement}
We provide a full code implementation of \methodabbr{}, including Novelty Prompting and CCL and OE training. We detail hyperparameters for our experiments in Section~\ref{sec:experimental_details}, prompt formats in Appendix~\ref{app:prompt_format}, and data processing details in Appendices~\ref{app:datasets} and \ref{app:tacred}. \methodabbr{} can be run with any text dataset and discriminative classifier model.
